Mathematical Modelling of TEAM and VTEAM Memristor Model Using VerilogA

Anyone who looks into the circuitry world will be familiar with the three fundamental circuit elements - capacitor, resistor, and inductor. These circuit elements are defined by the relation between two of the four fundamental circuit variables current, voltage, charge, and flux. However, in 1971, Prof. Leon Chua proposed on the grounds of symmetry that there should be a fourth fundamental circuit element that gives the relation between flux and charge. He named this the memristor, which is short for memory resistor. This theory was then practicallymodeled, in May 2008 when the researchers at HP Labs published a paper announcing a model for a physical realization of a memristor. This report mainly focuses on the model of memristor and its applications. The advantages of variable resistance, flexibility, no leakage current, and compatibility with CMOS. The element memristor exhibits different characteristics for different applications which results in the formation of different models of the memristor. This paper gives a review of different models of the memristor. Memristors devices can be used in many applications such as memory, logic, and neuromorphic systems. A computer model of the memristor would be a useful tool for analyzing circuit behavior to help in developing the application of this memristor is a passive circuit element via simulation. In this paper, various VerilogA model of memristor devices are simulated for sinusoidal inputs and output are verified Various window functions has been used. The circuit analysis of the various memristor models is done

==> ref.tex <==
 %
% Memristor simulation results
\subsection{Linear Ion Drift Model}

\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{Pictures/Linear/L3.jpg}
\caption{Linear Linear Ion Drift Model Results}
\label{Figure1a1b}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{Pictures/Linear/L2.jpg}
\caption{Linear Ion Drift model  - VI Characteristics}
\label{Figure1a1b}
\end{figure}

\subsection{Linear Ion Drift Model}

\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{Pictures/nonlinear/NL3.jpg}
\caption{Nonlinear Ion Drift Model Results}
\label{Figure1a1b}
\end{figure}


\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{Pictures/nonlinear/NL4.jpg}
\caption{Nonlinear Ion Drift model  - VI Characteristics}
\label{Figure1a1b}
\end{figure}

\subsection{Simmons Tunnel Barrier Model}

\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{Pictures/simmons/S3.jpg}
\caption{Simmons Tunnel Barrier Model Results}
\label{Figure1a1b}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{Pictures/simmons/S5.jpg}
\caption{Simmons Tunnel Barrier Model - VI Characteristics}
\label{Figure1a1b}
\end{figure}

\subsection{TEAM Model}
\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{Pictures/Team/T3.jpg}
\caption{TEAM Model Results}
\label{Figure1a1b}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{Pictures/Team/T5.jpg}
\caption{TEAM Model - VI Characteristics}
\label{Figure1a1b}
\end{figure}

\subsection{VTEAM Model}

\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{Pictures/VTeam/1Vteam.png}
\caption{VTEAM Model Results}
\label{Figure1a1b}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{Pictures/VTeam/2Vteam.png}
\caption{VTEAM Model Results}
\label{Figure1a1b}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{Pictures/VTeam/3Vteam.png}
\caption{VTEAM Model - VI Characteristics}
\label{Figure1a1b}
\end{figure}
